Closing the Gap Between Short and Long XORs for Model Counting

Many recent algorithms for approximate model counting are based on a reduction to combinatorial searches over random subsets of the space defined by parity or XOR constraints. Long parity constraints (involving many variables) provide strong theoretical guarantees but are computationally difficult. Short parity constraints are easier to solve but have weaker statistical properties. It is currently not known how long these parity constraints need to be. We close the gap by providing matching necessary and sufficient conditions on the required asymptotic length of the parity constraints. Further, we provide a new family of lower bounds and the first non-trivial upper bounds on the model count that are valid for arbitrarily short XORs. We empirically demonstrate the effectiveness of these bounds on model counting benchmarks and in a Satisfiability Modulo Theory (SMT) application motivated by the analysis of contingency tables in statistics.

==> SATCount.tex <==
\subsection{Model Counting Benchmarks}

%We also apply our method to the "central" \#P problem: SAT counting, or \#SAT. This family of problems seek to compute the number of satisfying assignments of a SAT formula. In particular, we consider SAT formulas encoded in standard CNF form. 
We evaluate the quality of our new bounds on a standard model counting benchmark (ANOR2011) from \namecite{kroc2011leveraging}. Both lower and upper bounds presented in the previous section are parametric: they depend both on $m$, the number of constraints, and $f$, the constraint density. Increasing $f$ is always beneficial, but can substantially increase the runtime. The dependence on $m$ is more complex, and we explore it empirically.
%\stefano{what's the right way to say this?}. 
To evaluate our new bounds, we consider a range of values for $f \in [0.01,0.5]$, %and use a simple approach that finds an $m$ with good promise with a handful of samples, and finish the algorithm on the $m$ that provides the best expected bound.
and use a heuristic approach to first identify a promising value for $m$ using a small number of samples $T$, and then collect more samples for that $m$ to reliably estimate $P[S(h)\geq 1]$ and improve the bounds on $|S|$. 
%Any $m$ has the promise to give us a bound, but it is obvious that not all values of m are worthy of exploring. 
%Our strategy chooses the next $m$ using an upper confidence style bound to balance exploration and exploitation. 
%In practice, the agent is capable of concentrating $1/2 ~ 1/3$ of its computational efforts in the optimal m it chooses.
%\shengjia{Feel free to remove this (Even though the experiments are indeed performed by bandit rather than exhaustive search, which may lead people to have incorrect expectation of how fast the SAT instances are solved)}

We primarily compare our results to ApproxMC \cite{chakraborty2013scalable}, which can compute a constant factor approximation to user specified precision with arbitrary confidence (at the cost of more computation time). ApproxMC is similar to SPARSE-COUNT, and uses long parity constraints. For both methods, Cryptominisat version 2.9.4~\cite{soos2009extending} is used as an NP-oracle $\mathcal{O}_S$ (with Gaussian elimination enabled), and the confidence parameter is set to $0.95$, so that bounds reported hold with $95\%$ probability.

Our results on the \emph{Langford12} instance (576 variables, 13584 clauses, $10^5 \approx \exp(11.5)$ solutions) are shown in Figure~\ref{fig:SATLB}. The pattern is representative of all other instances we tested. The tradeoff between quality of the bounds and runtime, which is governed by $f$, clearly emerges. Instances with small $f$ values can be solved orders of magnitude faster than with full length XORs ($f \approx 0.5$), but provide looser bounds. Interestingly, lower bounds are not very sensitive to $f$, and we empirically obtain good bounds even for very small values of $f$. 
We also evaluate ApproxMC (horizontal and vertical lines) with parameter setting of $\epsilon=0.75$ and $\delta=0.05$, obtaining an 8-approximation with probability at least $0.95$. The runtime is $47042$ seconds. It can be seen that ApproxMC and our bounds offer comparable model counts for dense $f \approx 0.5$. 
However, our method allows to trade off computation time against the quality of the bounds. 
We obtain non-trivial upper bounds using as little as $0.1\%$ of the computational resources required with long parity constraints, a flexibility not offered by any other method.


%At the same time, the bottom panel of the figure shows that increasing $f$ also makes the computational task much harder, thereby reinforcing the benefit of being able to derive provable upper bounds using very sparse constraints.

%Even though our method cannot compute a approximation to arbitrary precision, we do guarantee a constant factor approximation when $f$ approaches $f^*$. 

Table~\ref{table:SATCount} summarizes our results on other instances from the benchmark and compares them with ApproxMC with a 12 hour timeout.
%For some instances, ApproxMC is allowed to run slightly longer so that it does not time out. 
We see that for the instances on which ApproxMC is successful, our method obtains approximate model counts of comparable quality and is generally faster. While ApproxMC requires searching for tens or even hundreds of solutions during each iteration, our method needs only one solution per iteration. Further, we see that long parity constraints can lead to very difficult instances that cannot be solved, thereby reinforcing the benefit of being able to derive provable upper and lower bounds using very sparse constraints. Our method is designed to produce non-trivial bounds even when the computational budget is significantly limited, with bounds degrading gracefully with runtime. 

\FloatBarrier
\begin{figure}[ht]
    \centering
    \includegraphics[trim={5ex 5ex 5ex 14ex},clip,width=.95\columnwidth]{graph/log_bound_vs_time_v2}
    \caption{Log upper and lower bound vs. computation time. Point labels indicate the value of $f$ used.}
    \label{fig:SATLB}
\end{figure}


% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\columnwidth]{graph/bound_vs_f}
%     \caption{Log upper and lower bound vs. f}
%     \label{fig:SATBF}
% \end{figure}


\input{SATCountTable}


==> SATCountTable.tex <==
\begin{table*}[t]
\caption{Comparison of run time and bound quality on the ANOR2011 dataset. All true counts
%\footnote{The Langford CNF instances are the same as ANOR2011. The true counts for these instances, however, do not appear to correspond to the known analytic counts for the Langford problem at http://oeis.org/A014552/list.}
and bounds are in log scale.}
\label{table:SATCount}
\centering
\begin{small}
\begin{tabular}{|lcc|ccc|ccc|cc|}
\hline
 & Num. & True & \multicolumn{3}{c|}{Upper Bound} \Tstrut & \multicolumn{3}{c|}{Lower Bound} & \multicolumn{2}{c|}{ApproxMC} \\
SAT Instance & Vars. & Count & UB  & Runtime(s) & $f$ & LB & Runtime (s) & $f$ & Estimate & Runtime (s) \\
\hline
\Tstrut
% lang12 true count from http://oeis.org/A014552/list is 11.59; it may or may not correspond to this CNF instance
lang12         & 576  & -- & 14.96 & 19000 & 0.5 & 11.17 & 1280 & 0.1 & 12.25 & 47042 \\
wff.3.150.525  & 150  & 32.57 & 35.06 & 3800  & 0.5 & 31.69 & 3600 & 0.1  & 32.58 & 43571 \\
% lower bound 31/91 SAT, m=48
\hline
\Tstrut
2bitmax-6      & 252  & 67.52 & 69.72 & 355   & 0.5 & 67.17 & 1000 & 0.5  & -- & timeout \\
% lang15 true count from http://oeis.org/A014552/list is 19.60; doesn't correspond to this CNF instance
 lang15         & 1024 & -- & 352.5 & 240   & 0.02 & 19.58 & 6400 & 0.02 & -- & timeout \\
% lower bound 309/1806 SAT, m=31
ls8-normalized & 301  & 27.01 & 201.5 & 3800 & 0.02 & 25.34 & 3600 & 0.02 & -- & timeout \\
% lower bound 58/111 SAT, m=38
wff.3.100.150  & 100  & 48.94 & 51.00 & 2100  & 0.5 & 48.30 & 3600 & 0.5  & -- & timeout \\
wff.4.100.500  & 100  & --    & 69.31 & 1100  & 0.05 & 37.90 & 3600 & 0.05 & -- & timeout \\
% lower bound 150/2421 SAT, m=59
\hline
\end{tabular}
\end{small}
\end{table*}

==> abstract.tex <==
\begin{abstract}
\begin{comment}
The statistical analysis of contingency tables is an important problem in scientific data analysis. Approximate techniques based on sampling schemes are often used. These techniques, however, typically provide tight accuracy guarantees only in the limit. We present a new approach that is asymptotically accurate and also provides certificates in the form of lower and upper bounds on the statistics of interest. These bounds are generated in an anytime fashion and can be improved by increasing the computational budget. Our approach can leverage Satisfiability Modulo Theory solvers for the analysis of contingency table data subject to constraints that might encode prior domain knowledge. We show that our technique can provide accurate results and new bounds on several challenging real world datasets from the social sciences and ecology.
\end{comment}
Many recent algorithms for approximate model counting are based on a reduction to combinatorial searches over random subsets of the space defined by parity or XOR constraints. 
Long parity constraints (involving many variables) provide strong theoretical guarantees but are computationally difficult. Short parity constraints are easier to solve but have weaker statistical properties. It is currently not known how long these parity constraints need to be. We close the gap by providing matching necessary and sufficient conditions on the required asymptotic length of the parity constraints. Further, we provide a new family of lower bounds and the first non-trivial upper bounds on the model count that are valid for arbitrarily short XORs. We empirically demonstrate the effectiveness of these bounds on model counting benchmarks and in a Satisfiability Modulo Theory (SMT) application motivated by the analysis of contingency tables in statistics.	
\end{abstract}


==> asymptotic_bound.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
\section{Asymptotically Optimal Constraint Density}

\newcommand\minf{\tilde{f}}

We analyze the asymptotic behavior of the minimum constraint density $f$ needed for SPARSE-COUNT to produce correct bounds with high confidence. As noted earlier, the bottleneck lies in ensuring that $f$ is large enough for a randomly chosen hash bin to receive at least one element of the set $S$ under consideration, i.e., the hash family shatters $S$.

\begin{mydef}
Let $n,m \in \mathbb{N}$. For any fixed $\epsilon > 0$, the \emph{minimum constraint density} $f = \minf_\epsilon(m,n)$ is defined as the pointwise smallest function such that for any constant $c \geq 2$, $\mathcal{H}^f_{m \times n}$ $\epsilon$-shatters all sets $S \in \{0,1\}^n$ of size $2^{m+c}$.
\end{mydef}

We will show (Theorem~\ref{thm:asymp}) that for any $\epsilon > 0$, $\minf_\epsilon(m,n) = \Omega(\frac{\log m}{m})$, and this is asymptotically tight when $\epsilon$ is small enough and $m = \Theta(n)$, which in practice is often the computationally hardest regime of $m$. Further, for the regime of $m = \Theta(n^\beta)$ for $\beta < 1$, we show that $\minf_\epsilon(m,n) = \bigOh(\frac{\log^2 m}{m})$. Combined with the observation that $\minf_\epsilon(m,n) = \Theta(1)$ when $m = \Theta(1)$, our results thus reveal how the minimum constraint density evolves from a constant to $\Theta(\frac{\log m}{m})$ as $m$ increases from a constant to being linearly related to $n$.

The \emph{minimum average constraint length}, $n \cdot \minf_\epsilon(m,n)$, correspondingly decreases from $n/2$ to $\bigOh(n^{1-\beta} \log^2 n)$ to $\Theta(\log n)$, showing that in the computationally hardest regime of $m = \Theta(n)$, the parity constraints can in fact be represented using only $2^{\Theta(\log n)}$, i.e., a polynomial number of SAT clauses. %Theorem~\ref{thm:asymp} in fact shows that one needs at most $\bigOh(n^3)$ SAT clauses per parity constraint in this regime.

% We now purpose an asymptotic guarantee for the minimum but adequate $f^*$ for which we can obtain a constant factor approximation. Namely we show that if $m=\Theta(n)$, $f^*$ scales with $\Theta(\frac{\log{m}}{m})$, and if $m=\Theta(n^{\beta}), \beta < 1$, $f^*$ scales with at most $\bigOh(\frac{\log^2{m}}{m})$. We also show that the constant in the asymptotic bound is no greater than a small constant. This is highly desirable because sparse WISH or algorithms with similar spirits can be shown to compute counting problems such as \#SAT with tens of thousands of variables. An asymptotic guarantee on the scale of $\frac{\log{m}}{m}$ for n on this scale could mean that $f^*$ can be tens of times sparser than $\half$. Furthermore, the resulting average constraint length is $O(\log n)$. This implies that each constraint can be represented with $O(2^{\log n}) = O(n)$ clauses. \ashish{This would be $2^{\bigOh(\log n)} = n^{\bigOh(1)}$, i.e., a polynomial, not necessarily linear.} \par

% Formally We give the following main theorem, then we give a sketch on how they can be proved, leaving the details in the appendix \par

\begin{theorem}
\label{thm:asymp}
% For the family $H \in \mathcal{H}^f$, let $f^*$ be the minimum constraint density so that for any $c \geq 2$, for any set $S$ with size $2^{m+c}$, and for any $2 < \delta < 5$, we can have $Pr \lbrace S(h) \geq 1 \rbrace \geq 1 - \frac{1}{\delta} $. Then:
The minimum constraint density, $\minf_\epsilon(m,n)$, behaves as follows:
\begin{enumerate}
\item Let $\epsilon > 0$. For any $k < 1$, there exists $m_k$ such that for all $m > m_k$:
%\[ \limn \minf(m,n) \geq \frac{\log{m}}{m}\]
\[ \minf_\epsilon(m,n) > k \frac{\log{m}}{m}\]
In other words, $\limm \minf_\epsilon(m,n) \geq \frac{\log m}{m}$.
\item Let $\epsilon \in (0,\frac{3}{10})$ and $\alpha \in (0,1)$. For $m = \alpha n$:
\[ \limn \minf_\epsilon(m,n) \leq (\kbound) \frac{\log{m}}{m} \]
\item Let $\epsilon \in (0,\frac{3}{10})$ and $\alpha, \beta \in (0,1)$. For $m = \alpha n^\beta$:
\[ \limn \minf_\epsilon(m,n) \leq \frac{1-\beta}{2\beta}\frac{\log^2{m}}{m} \]
\end{enumerate}
\end{theorem}

% There are two important conclusions that can be immediately derived from Theorem~\ref{thm:asymp}.

% 1. The bounds are matching when $m = \Theta(n)$, and we have 
% \[ f^* = \Theta \left(\frac{\log{m}}{m}\right) \]
% however, when $m = \Theta(n^{\beta})$ for $0 < \beta < 1$, whether the bound can be matching is a question we leave open. \par 

%\ashish{unsure; revisit} By Theorem~\ref{thm:const}, the $f^*$ that satisfies Theorem~\ref{thm:asymp} can give a $(4 + \eta)$- approximation for any $\eta > 0$ in Algorithm~\ref{algo_wish}

The lower bound in Theorem~\ref{thm:asymp} follows from analyzing the shattering probability of an $m+c$ dimensional hypercube $S_c=\{x \mid x_j = 0 \ \ \forall j > m+c\}$. Intuitively, random parity constraints of density smaller than $\frac{\log m}{m}$ do not even touch the $m+c$ relevant (i.e., non-fixed) dimensions of $S_c$ with a high enough probability, and thus cannot shatter $S_c$ (because all elements of $S_c$ would be mapped to the same hash bin).

For the upper bounds, we exploit the fact that $\minf(m,n)$ is at most the $f^*$ function introduced by \namecite{ermon2014low} and provide an upper bound on the latter. Intuitively, $f^*$ was defined as the minimum function such that the variance of $S(h)$ is relatively small. The variance was upper bounded by considering the worst case ``shape'' of $|S|$: points packed together unrealistically tightly, all fitting together within Hamming distance $w^*$ of a point. For the case of $m = \alpha n$, we observe that $w^*$ must grow as $\Theta(n)$, and divide the expression bounding the variance into two parts: terms corresponding to points that are relatively close (within distance $\lambda n$ for a particular $\lambda$) are shown to contribute a vanishingly small amount to the variance, while terms corresponding to points that are farther apart are shown to behave as if they contribute to $S(h)$ in a pairwise independent fashion. The $\frac{\log m}{m}$ bound is somewhat natural and also arises in the analysis of the rank of sparse random matrices and random sparse linear systems~\cite{kolchin1999random}. For example, this threshold governs the asymptotic probability that a matrix $A$ generated as in Definition \ref{def:sparse-hash} has full rank~\cite{cooper2000rank}. The connection arises because in our setting, the rank of the matrix $A$ affects the quality of the hashing. For example, an all-zero matrix $A$ (of rank $0$) would map all points to the same hash bin.  
%\ashish{``intuition" becoming too loose/incorrect?}
%\ashish{Should connect to the full-rank business and add some refs. Stefano?}


==> conclusion.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%
\section{Conclusions}
%%%%%%%%%%%%%%%%%%%%%%%%

We introduced a novel analysis of the randomized hashing schemes used by numerous recent approximate model counters and probabilistic inference algorithms. We close a theoretical gap, providing a tight asymptotic estimate for the minimal constraint density required. Our analysis also shows, for the first time, that even very short parity constraints can be used to generate non-trivial upper bounds on model counts. Thanks to this finding, we proposed a new scheme for computing anytime upper and lower bounds on the model count. Asymptotically, these bounds are guaranteed to become tight (up to a constant factor) as the constraint density grows. Empirically, given very limited computational resources, we are able to obtain new upper bounds on a variety of benchmarks, including a novel application for the analysis of statistical contingency tables.

A promising direction for future research is the analysis of related ensembles of random parity constraints, such as low-density parity check codes~\cite{achlioptasstochastic}. 

% As an application, we consider the challenging problem of counting contingency tables, a very important problem in scientific data analysis. We introduce an approach that uses a Satisfiability Modulo Theory (SMT) encoding to analyze the tables. Our approach allows us to naturally incorporate additional constraints on the tables imposed by prior domain knowledge, such as certain entries being forced to be zero or within a certain range. We demonstrate the effectiveness of our approach on a range of real world datasets.


==> experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experimental Evaluation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\input{SATCount}
% \subsection{Counting Contingency Tables}

% We consider the analysis of contingency tables subject to domain specific constraints, including structural zeros~\cite{chen2007conditional} (i.e., certain entries of the table are required to be $0$) in a variety of domains. For each dataset, the input consists of $r$ row marginals and $c$ column marginals. Some datasets require binary contingency tables, i.e., $\{0,1\}$ entries. $S$ denotes the set of all possible contingency tables that respect the given marginals and other constraints. The goal is to compute provable bounds on $\log_2 |S|$. We begin with a description of the datasets.

%\input{smt_contingency}
\input{smt_contingency_shorter}
We evaluate our bounds on six datasets:

\textbf{Darwin's Finches (df).}
%
The marginals for this binary contingency table dataset are from \citet{chen2005sequential}. This is one of the few datasets with known ground truth: $\log_2 |S| \approx 55.8982$, found using a clever divide-and-conquer algorithm of David desJardins. 
%The corresponding ideal value is thus $i^* = \log_2 |S| = 55.8982$. 
The 0-1 label in cell $(x, y)$ indicates the presence or absence of one of 13 finch bird species $x$ at one of 17 locations $y$ in the Gal\'apagos Islands. To avoid trivialities, we drop one of the species that appears in every island, resulting in $12 \times 17 = 204$ binary variables.
%The name ``Darwin's finches'' reflects the fact that some of these species were collected by Charles Darwin when he visited the Gal\'apagos. In ecology, researchers are interested in Fisher's test to decide whether the distribution of finches in these islands is an effect of chance events in the distant past or the result of competition.

\textbf{Climate Change Perceptions (icons).}
%
This $9 \times 6$ non-binary dataset is taken from the \texttt{alymer} \texttt{R} package \cite{west2008exact}. It concerns lay perception of climate change. The dataset is based on a study reported by \citet{oneil2008:thesis} in which human subjects are asked to identify which icons (such as polar bears) they find the most concerning. There are 18 structural zeros representing that not all icons were shown to all subjects.

\textbf{Social Anthropology (purum).}
%
This $5 \times 5$ non-binary dataset~\cite{west2008exact} concerns marriage rules of an isolated tribe in India called the Purums, which is subdivided into $5$ sibs. Structured zeros represent marriage rules that prevent some sibs from marrying other sibs. %, resulting in structured zero constraints in the table.

\textbf{Industrial Quality Control (iqd).}
%
This $4 \times 7$ non-binary dataset~\cite{west2008exact} captures an industrial quality control setting. Cell $(x,y)$ is the number of defects in the $x$-th run attributable to machine $y$. It has 9 structured zeros, representing machines switched off for certain runs.

\textbf{Synthetic Data (synth).}
%
This $n \times n$ binary dataset contains \emph{blocked matrices}~\cite{golshan2013row}. The row and column marginals are both $\{1,n-1, \ldots, n-1\}$. It can be seen that a blocked matrix has either has a value of 1 in entry $(1, 1)$ or it has two distinct entries with value 1 in the first row and the first column, cell $(1, 1)$ excluded. Instantiating the first row and the first column completely determines the rest of the table. It is also easy to verify that the desired count is $1+(n-1)^2$.


\begin{table}[t]
\caption{Lower (LB) and upper (UB) bounds on $\log_2 |S|$.
%\textsc{synth}\_8 is the synthetic dataset with $n=8$.
The trivial upper bound (Trv.~UB) is the number of binary variables. $f^\ast$ denotes the best previously known minimum $f$ \cite{ermon2014low} required for provable upper bounds.}
\label{summary-table}
%\vskip 0.15in
\centering
\begin{small}
%\begin{sc}
%\begin{tabular}{p{0.8in}p{0.5in}p{0.5in}p{0.5in}p{0.5in}}
\addtolength{\tabcolsep}{-0.7ex}
\begin{tabular}{lcc|rrrr}
\hline
%\abovespace
\Tstrut
Dataset & Table Size & $f^\ast$ & LB ($f$) & $\log_2 |S|$ & UB & Trv.~UB\\
%\belowspace
\hline
%\abovespace
%df  \Tstrut  & 12 $\times$ 17  & 0.18 & {\bf 55} (0.03) & 55.90 & {\bf 150} & 204 \\
df  \Tstrut  & 12 $\times$ 17  & 0.18 & {\bf 53} (0.03) & 55.90 & {\bf 150} & 204 \\
icons & 9 $\times$ 6    & 0.19 & {\bf 58} (0.04) & - & {\bf 183} & 236 \\
purum & 5 $\times$ 5    & 0.26 & {\bf 29} (0.13) & - & {\bf 52}  & 125 \\
iqd   & 4 $\times$ 7    & 0.34 & {\bf 15} (0.10) & - & {\bf 17}  & 76  \\
synth\_8 & 8 $\times$ 8 & 0.41 & {\bf 5}  (0.30) & 5.64 & {\bf 16} & 64\\
%\belowspace
synth\_20 & 20 $\times$ 20 & 0.42 & {\bf 8} (0.40) & 8.49 & {\bf 14} & 400\\
\hline
\end{tabular}
%\end{sc}
\end{small}
%\vskip -0.1in
\end{table}


%\subsection{Counting Contingency Tables}

Table \ref{summary-table} summarizes the obtained lower and upper bounds on the number of contingency tables, with a 10 minute timeout. For the datasets with ground truth, we see that very sparse parity constraints (e.g., $f=0.03$ for the Darwin finches dataset, as opposed to a theoretical minimum of $f^*=0.18$) often suffice in practice to obtain very accurate lower bounds. For the iqd dataset, we obtain upper and lower bounds within a small constant factor. For other datasets, there is a wider gap between the upper and lower bounds. However, the upper bounds we obtain are orders of magnitude tighter than the trivial log-upper bounds, which is the number of variables in a binary encoding of the problem. % of the corresponding counting problem.
%Note that trying to get an upper bound on the number of valid contingency tabled using a lower bound on  what is NOT a valid table is hopeless. 

%\subsection{Tables with additional constraints}
%Use Purum tribes as an example.

% \subsection{Computation vs.\ Accuracy Tradeoff}

% \begin{figure}[tb]
% \centering
% \includegraphics[scale=0.45,trim=0ex 0ex 0ex 5ex,clip]{plots/f_vs_bound_quality}
% \vskip 0.15in
% \includegraphics[scale=0.45,trim=0ex 0ex 0ex 7ex,clip]{plots/f_vs_runtime}
% \caption{Impact of increasing $f$ on (top) the quality of upper and lower bounds on $\log_2 |S|$ and (bottom) computational time}
% \label{fig:f_vs_bound_quality_and_runtime}
% \end{figure}

% As mentioned earlier, our method allows one to trade off computation time against the quality of lower and upper bounds. The larger the constraint sparsity $f$, the more computational resources one typically needs in order to compute bounds on $|S|$. The top panel of Figure~\ref{fig:f_vs_bound_quality_and_runtime} shows how the obtained bounds for the Darwin's finches dataset improve as $f$ is increased from $0.014$ to $0.044$. The lower bound approaches the ground truth fairly quickly, while the upper bound continues to get tighter. At the same time, the bottom panel of the figure shows that increasing $f$ also makes the computational task much harder, thereby reinforcing the benefit of being able to derive provable upper bounds using very sparse constraints.



==> introduction.tex <==
%%%%%%%%%%%%%%%%%%
\section{Introduction}

\js{can probably cut first paragraph.  I think it would be better if you define your task of interest up-front.
i don't know what a contingency table / chi-squared test is, e.g. like, i'd roughly start with what's currently paragraph 3
except before that, set up the task talk about why it's hard
and how you'll solve it. citations are good here, too
you don't need to talk about probability being good / probabilistic inference being hard, because everyone at ICML already agrees with that (although it being hard for this particular task is worth discussing)}

\begin{comment}
Probabilistic models are the cornerstone of statistical machine learning. Probability theory provides the mathematical foundation to model our beliefs and to update them as new evidence is obtained. A typical computation is to compute a posterior probability given evidence in order to make a prediction. In statistical \emph{hypothesis testing}, in order to calculate the significance of the observed data, we often have to compute the probability of observing data as extreme, or relatively more extreme if the null hypothesis is true. 
Both of these tasks, along with many other similar probabilistic inference tasks, are very challenging from the computational point of view~\cite{roth1996hardness}. While the problem can be easily solved in certain simple probabilistic models, it becomes extremely difficult for larger and richer statistical models, capturing complex interactions between thousands of variables.
\end{comment}

%In scientific data analysis problems, it is often necessary to answer these probabilistic inference queries very accurately, for instance, when we have to compute a p-value to decide whether or not we should reject a null hypothesis~\cite{fisher1954,fh1951:contingency}. Unfortunately, traditional approximate inference techniques~\cite{madras2002lectures,andrieu2003introduction,jordan1999introduction} only provide asymptotic guarantees, unless the underlying model satisfies some rather restrictive special conditions like low-treewidth or fast mixing times~\cite{jerrum1997markov}.
%In the general case, there is usually no information about the quality of the approximation obtained. Sampling based techniques, for example, might completely miss an important area of the state space. 
%In the past 25 years, combinatorial search and optimization technology has made tremendous progress. 

Model counting is the problem of computing the number of distinct solutions of a given Boolean formula. It is a classical problem that has received considerable attention from a theoretical point of view~\cite{valiant1979complexity,stockmeyer1985approximation}, as well as from a practical perspective~\cite{sang2004combining,gogate2007approximate}. Numerous probabilistic inference and decision making tasks, in fact, can be directly translated to (weighted) model counting problems~\cite{richardson2006markov,gogate2011probabilistic}. As a generalization of satisfiability testing, the problem is clearly intractable in the worst case. Nevertheless, there has been considerable success in both exact and approximate model counting algorithms, motivated by a number of applications~\cite{sang2005solving}. 

Recently, approximate model counting techniques based on randomized hashing have emerged as one of the leading approaches~\cite{mbound,cav13,ermon2014low,ivrii2015computing,achlioptasstochastic,belle2015hashing}. While approximate, these techniques provide strong guarantees on the accuracy of the  results in a probabilistic sense. Further, these methods all reduce model counting to a small number of combinatorial searches on a randomly projected version of the original formula,
%This projection is always implemented by augmenting the original formula
obtained by augmenting it with randomly generated parity or XOR constraints.
%~\cite{mbound,cav13,ermon2014low,ivrii2015computing,achlioptasstochastic,belle2015hashing}.
This approach allows one to leverage decades of research and engineering in combinatorial reasoning technology, such as fast satisfiability (SAT) and SMT solvers~\cite{biere2009handbook}. 
%Consistently with worst-case computational complexity hardness results on inference, these search problems are difficult to solve in the worst case. 
%Luckily, real world models typically do not represent the worst-case scenario, and when these problems \emph{can} in fact be solved, these techniques provide a \emph{certificate} that the results obtained are accurate.

%At the same time, randomized hashing techniques produce combinatorial search problems that we could not solve using state-of-the-art technology. 
While modern solvers have witnessed tremendous progress over the past 25 years, model counting techniques based on hashing tend to produce instances that are difficult to solve. In order to achieve strong (probabilistic) accuracy guarantees, existing techniques require each randomly generated parity constraint to be relatively long, involving roughly half of the variables in the original problem. Such constraints, while easily solved in isolation using Gaussian Elimination, are notoriously difficult to handle when conjoined with the original formula. Shorter parity constraints, i.e., those involving a relative few variables, are much more easily handled by SAT solvers, but their statistical properties are not well understood~\cite{ghss07:shortxors}.

Recently, \citet{ermon2014low} showed that long parity constraints are not strictly necessary, and that one can obtain the \emph{same accuracy guarantees} using shorter XORs, which are computationally much more friendly. They provided a closed form expression, allowing an easy computation of an XOR length that suffices, given various parameters such as the number of problem variables, the number of constraints being added, and the size of the solution space under consideration. It is, however, currently now known how tight their sufficiency condition is, how it scales with various parameters, or whether it is in fact a necessary condition.
%It is, however, currently not known exactly  how long the parity constraints need to be. 

\emph{We resolve these open questions by providing an analysis of the optimal asymptotic constraint length} required for obtaining high-confidence approximations to the model count. Surprisingly, for formulas with $n$ variables, we find that when $\Theta(n)$ constraints are added, a constraint length of $\Theta(\log n)$ is both necessary and sufficient. This is a significant improvement over standard long XORs, which have length $\Theta(n)$. Constraints of logarithmic length can, for instance, be encoded efficiently with a polynomial number of clauses. We also study how the sufficient constraint length evolves from $\bigOh(\log n)$ to $\bigOh(n^\gamma \log^2 n)$ to $n/2$ across various regimes of the number of parity constraints.

As a byproduct of our analysis, we obtain a \emph{new family of probabilistic upper and lower bounds that are valid regardless of the constraint length} used. These upper and lower bounds on the model count reach within a constant factor of each other as the constraint density approaches the aforementioned optimal value. The bounds gracefully degrade as we reduce the constraint length and the corresponding computational budget. While lower bounds for arbitrary XOR lengths were previously known~\cite{ghss07:shortxors,uai13LPCount}, this is the first non-trivial upper bound in this setting. Remarkably, even though we rely on random projections and therefore only look at subsets of the entire space (a \emph{local} view, akin to traditional sampling), we are able to say something about the \emph{global} nature of the space, i.e., a probabilistic upper bound on the number of solutions.

% It has been previously suggested that one can trade-off the difficulty of the resulting combinatorial search problems with the quality of the approximation obtained for the model counting problem. In particular, one can trade-off the statistical efficiency of the randomized hashing to reduce the runtime. These techniques provide lower bounds on the counts which are empirically very good, but the upper bound part is lost. 

% We are therefore in a binary situation where statistical efficient hash functions would provide matching (within a constant factor) upper and lower bounds, but lead to combinatorial search problems that are too hard to solve. Weaker hash functions, on the other hand, lead to easy combinatorial search problems but do not provide \emph{any} upper bound. In this paper, we provide a novel analysis that provides lower \emph{and} upper bounds that gracefully degrade as we weaken the hash functions used, i.e. reduce the runtime of the technique. Our result is very surprising because even though we rely on random projections and therefore only look at subsets of the entire space (a \emph{local} view, like in a traditional sampling technique), we are able to say something about the \emph{global} nature of the space. Intuitively, we can provide (probabilistic) guarantees that even though we take a local view through samples, we cannot have missed (sufficiently) important regions of the space. Intuitively, hashing based techniques can provide upper bounds because they effectively consider exponentially large sets of configurations, exploiting randomness amplification ideas. We therefore provide an anytime approach, where one can obtain lower and upper bounds for any given computational budget, with a guarantee that given enough computational budget, these bounds will eventually be tight (within a constant factor). We therefore provide asymptotic guarantees like other sampling techniques.

We evaluate these new bounds on standard model counting benchmarks and on a new counting application arising from the analysis of contingency tables is statistics. These data sets are common in many scientific domains, from sociological studies to ecology~\cite{sheldon2011collective}. We provide a new approach based on SMT solvers and a bit-vector arithmetic encoding. Our approach scales very well and produces accurate results on a wide range of benchmarks. 
%In scientific data analysis problems, it is often necessary to answer these probabilistic inference queries very accurately, for instance, when we have to compute a p-value to decide whether or not we should reject a null hypothesis~\cite{fisher1954,fh1951:contingency}.
It can also handle additional constraints on the tables, which are very common in scientific data analysis problems, where prior domain knowledge translates into constraints on the tables (e.g., certain entry must be zero because the corresponding event is known to be impossible). 
% While sampling techniques can be developed for certain types of constraints, they usually require the manual design of constraint-specific Markov Chains or proposal distributions with certain desired properties (e.g., using Groebner basis analysis to ensure ergodicity).
% In contrast, our technique is very general and can directly support a wide range of constraints.
We demonstrate the capability to handle structural zeroes~\cite{chen2007conditional} in real experimental data.

\begin{comment}
Our work is motivated by the statistical analysis of contingency tables. As a running example, we will consider Fisher's exact test, a statistical significance test used in the analysis of contingency tables~\cite{fisher1954,fh1951:contingency}. 
While a computationally efficient chi-squared test approximation can be used in certain cases, computing a p-value according to Fisher's exact test is computationally very difficult for high dimensional contingency tables. Intuitively, one has to compute a (weighted) count of a combinatorially large number of possible contingency tables that are consistent with given fixed row and column marginals. Monte Carlo approximations, including specialized importance sampling and MCMC, have been developed. Importance sampling~\cite{chen2005sequential} and MCMC~\cite{diaconis1998algebraic,diaconis1995rectangular}  are often quite accurate, but it's not typically possible to verify if the results are accurate or not. These techniques are typically evaluated on synthetic or small data sets for which ground truth is known. However, these techniques only provide accuracy guarantees in the limit. 
\end{comment}

% STORY:\\
% - probabilistic inference is a key computational problem, e.g. posteriors, expectations, hypothesis testing\\
% - scientific domains, we need accuracy guarantees: e.g., compute a p-value, accept or reject a null hypothesis. fisher's exact test for example. mention Darwin's finches data set \\
% - traditional techniques only provide asymptotic guarantees, unless trees,fast mixing, etc\\
% - recent approaches based on hashing + combinatorial search provide tight guarantees. however, need statistically good hash functions. otherwise provide only lower bounds. \\
% - we tried applying this to contingency tables, cannot be solved using combinatorial search. lower bounds based on sparse constraints are empirically good, but again unsatisfactory. we want to know if the answers are accurate or not.\\
% - novel analysis: provides anytime upper bounds. very surprising. even though we sample "locally", we can still say something "global"\\
% - apply to contingency tables. use modern theorem proving technology, SMT solvers. propositional logic plus additional theories
% - natively handles constraints. for example, structured zeros\\
% - works well in practice\\


% In ICML-2014~\cite{wishicml13,ermon2014low}, it is shown that the pairwise independence is not strictly
% necessary, because it is sufficient to find statistically weaker hash
% functions that provide the same guarantees (up to an arbitrarily small
% error). 

% sampling techniques: generally no way of obtaining upper bounds. one might have completely missed an important area of the state space. hashing based techniques can provide upper bounds because they effectively consider exponentially large sets of configurations, exploiting randomness amplification ideas. 



==> smt_contingency.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Satisfiability Modulo Theory for\\ the Analysis of Contingency Tables}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Contingency Tables and Fisher's Exact Test}

In statistics, a \emph{contingency table} is a matrix that captures the (multivariate) frequency distribution of two variables with $r$ and $c$ possible values, resp. E.g., if the variables are gender (male or female) and handedness (left- or right-handed), then the corresponding $2 \times 2$ contingency table has frequencies for the four possible value combinations. Such a table is associated with $r$ row sums and $c$ column sums, also known as the row and column marginals, resp.

Fisher's exact test \cite{fisher1954,fh1951:contingency} tests contingency tables for homogeneity of proportion. Given fixed row and column marginals, it computes the probability of observing the entries found in the table under the null hypothesis that the distribution across rows is independent of the distribution across columns. This exact test, however, quickly becomes intractable for higher-dimensional tables or when $r$ and $c$ become very large. Statisticians, therefore, often resort to approximate significance tests, such as the chi-squared test.

The computational difficulty in performing Fisher's exact test is captured by the following counting question: \emph{Given $r$ row marginals and $c$ column marginals, how many $r \times c$ integer matrices $M$ are there with these row and column marginals?} When entries of $M$ are restricted to be in $\{0,1\}$, the corresponding contingency table is called binary or Boolean. We are interested in counting both binary and integer contingency tables.

The techniques we described in the previous section are very general, and can be used to estimate the size of any subset $S$ for which we have a membership oracle. While the accuracy guarantees do not rely in any way on the actual implementation of the membership oracle, the runtime is effectively entirely determined by the time required to test membership subject to randomly generated (sparse) parity constraints. Technically, the membership queries are in NP, hence any solver for an NP-complete language can be used. The runtime heavily depends on the choice of the language and the problem encodings. Most of the previous applications have relied on CNF Satisfiability (SAT)~\cite{ermon2014low,cav13,mbound}, Integer Linear Programming (ILP)~\cite{uai13LPCount}, and Constraint Optimization (CP) solvers~\cite{wishicml13,gomes2007xors-csp}.

For the analysis of contingency tables, the domain can be naturally represented using integer arithmetic. Given a vector of $r$ integer, non-negative row marginals $R \in \mathbb{N}^r$ of and $c$ integer, non-negative column marginals $C \in \mathbb{N}^c$, the set of contingency tables consistent with these marginals and that we want to enumerate is defined as $S = \{A \in \mathbb{N}^{r\times x}: \sum_j A_{ij} = R_i,\sum_i A_{ij} = C_i \}$. These pseudoboolean constraints cannot be represented directly in CNF form (conjunction of disjunctions of variables), and would require encoding the arithmetic circuits with additional variables and constraints. The problem can be easily encoded as an ILP. Unfortunately, ILP solvers are typically designed to solve optimization problems and not feasibility queries. We therefore propose the encode the problem using a Satisfiability Modulo Theory (SMT) framework~\cite{BarST-SMTLIB}. SMT is powerful modeling framework that extends propositional logic with other underlying theories, e.g. bitvectors and real arithmetic. We choose to use a bitvector encoding where each entry $a_ij$ is represented as a bitvector of size $\lceil \log_2 \min(\min_k a_{ik},\min_\ell a_{\ell j}) \rceil$. The parity constraints used to implement hash functions are then randomly generated over the individual bits of each bitvector, and natively encoded into the model as XORs (without converting them into linear equations or clausal form). As a solver, we use the Z3 theorem prover from Microsoft Research~\cite{de2008z3}.


==> smt_contingency_shorter.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Satisfiability Modulo Theory for\\ the Analysis of Contingency Tables}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Contingency Tables and Fisher's Exact Test}

\subsection{SMT Models for Contingency Table Analysis}

In statistics, a \emph{contingency table} is a matrix that captures the (multivariate) frequency distribution of two variables with $r$ and $c$ possible values, resp. For example, if the variables are gender (male or female) and handedness (left- or right-handed), then the corresponding $2 \times 2$ contingency table contains frequencies for the four possible value combinations, and is associated with $r$ row sums and $c$ column sums, also known as the row and column marginals.

Fisher's exact test \cite{fisher1954} tests contingency tables for homogeneity of proportion. Given fixed row and column marginals, it computes the probability of observing the entries found in the table under the null hypothesis that the distribution across rows is independent of the distribution across columns. This exact test, however, quickly becomes intractable as $r$ and $c$ grow. Statisticians, therefore, often resort to approximate significance tests, such as the chi-squared test.

The associated counting question is: \emph{Given $r$ row marginals $R_i$ and $c$ column marginals $C_j$, how many $r \times c$ integer matrices $M$ are there with these row and column marginals?} When entries of $M$ are restricted to be in $\{0,1\}$, the corresponding contingency table is called binary. We are interested in counting both binary and integer tables.

This counting problem for integer tables is \#P-complete even when $r$ is 2 or $c$ is 2~\cite{dyer1997sampling}. Further, for binary contingency tables with so-called structural zeros~\cite{chen2007conditional} (i.e., certain entries of $M$ are required to be $0$), we observe that the counting problem is still \#P-complete. This can be shown via a reduction from the well-known \emph{permanent} computation problem, which is \#P-complete even for 0/1 matrices~\cite{valiant1979permanent}. 
%% temporarily commenting out to save space
\begin{comment}
Given an $n$-dimensional 0/1 matrix $\tilde{M}$, its permanent $\mathit{perm}(\tilde{M})$ is simply the number of ways one can select $n$ of the 1 entries of $\tilde{M}$ such that every row and every column is covered. To reduce this to a contingency table counting problem, create an $n \times n$ matrix $M$ with structural zeros in cells where $\tilde{M}$ has zeros. The number of possible contingency tables corresponding to $M$ when all row and column marginals are one is then precisely $\mathit{perm}(M)$.
\end{comment}

Model counting for contingency tables is formulated most naturally using integer variables and arithmetic constraints for capturing the row and column sums. While integer linear programming (ILP) appears to be a natural fit, ILP solvers do not scale very well on this problem as they are designed to solve optimization problems and not feasibility queries. We therefore propose to encode the problem using a Satisfiability Modulo Theory (SMT) framework~\cite{BarST-SMTLIB}, which extends propositional logic with other underlying theories, such as bitvectors and real arithmetic. We choose a bitvector encoding where each entry $a_{ij}$ of $M$ is represented as a bitvector of size $\lceil \log_2 \min(R_i, C_{j}) \rceil$. The parity constraints are then randomly generated over the individual bits of each bitvector, and natively encoded into the model as XORs. %(without converting them into linear equations or clausal form). 
As a solver, we use Z3~\cite{de2008z3}.


==> sparse_bounds.tex <==
%%%%%%%%%%%%%%%%%%%%%%
\section{Improved Bounds on the Model Count}

In the previous sections, we established the optimal (smallest) constraint density that provides a constant factor approximation on the model count $|S|$.
%, meeting the conditions of Theorem \ref{thm:const}. 
However, depending on the size and structure of $S$, even adding constraints of density $f^\ast\ll 0.5$ can lead to instances that cannot be solved by modern SAT solvers (see Table \ref{table:SATCount} below). 

In this section we show that for $f < f^\ast$ we can still obtain probabilistic upper and lower bounds. The bounds constitute a trade off between small $f$ for easily solved NP queries and $f$ close to $f^*$ for guaranteed constant factor approximation.

%\js{high-level comment: you probably want to put in more prose to 
%explain all the math here (in case you weren't already planning to)}
To facilitate discussion, we define $S(h) = |\{x \in S \mid h(x) = 0\}| = |S \cap h^{-1}(0)|$ to be the random variable indicating how many elements of $S$ \emph{survive} $h$, when $h$ is randomly chosen from $\mathcal{H}^f_{m \times n}$ as in Definition \ref{def:sparse-hash}.
Let $\mu_S = \Exp[S(h)]$ and $\sigma^2_S = \mathrm{Var}[S(h)]$.
%where $h$ is a hash function drawn (implicitly) from $\mathcal{H}^f_{m \times n}$ for some $f \in [0,1/2]$. 
Then, it is easy to verify that irrespective of the value of $f$, $\mu_S = |S|2^{-m}$. $\mathrm{Var}[S(h)]$ and $\Pr[S(h) \geq 1]$, however, do depend on $f$.

% \tum{this proposition seems to come from nowhere. If we're going to include it we might want to include proof in the appendix section too.}
% \begin{proposition}
% For $f \in [0,1/2]$ and $h \in_R \mathcal{H}^f_{m \times n}$, $\Pr[S(h) \geq 1]$ is a decreasing function of $m$.
% \end{proposition}


% \begin{mydef}
% \label{def:shatter}
% A family of hash functions $\mathcal{H}$ $\epsilon$-\emph{shatters} $S$ if $\Pr[S(h) \geq 1] \geq 1/2+\epsilon$ when $h \in_R \mathcal{H}$.
% \end{mydef}

%% commenting out, this seems to be never used...
% \begin{lemma}
% \label{lemma:shatter}
% If $\sigma_S \leq \mu_S / \sqrt{\frac{1/2+\epsilon}{1/2-\epsilon}}$, then $\mathcal{H}$ $\epsilon$-shatters $S$.
% \end{lemma}


%%%%%%
\subsection{Tighter Lower Bound on $|S|$}

Our lower bound is based on Markov's inequality and the fact that the mean of $S(h)$, $\mu_S = |S|2^{-m}$, has a simple relationship to $|S|$. Previous lower bounds~\cite{ghss07:shortxors,uai13LPCount} are based on the observation that if at least half of $T$ repetitions of applying $h$ to $S$ resulted in some element of $S$ surviving, there are likely to be at least $2^{m-2}$ solutions in $S$. Otherwise, $\mu_S$ would be too small (specifically, $\leq 1/4$) and it would be unlikely to see solutions surviving often. Unlike previous methods, we not only check whether the estimated $\Pr[S(h) \geq 1]$ is at least $1/2$, but also consider an empirical estimate of $\Pr[S(h) \geq 1]$. This results in a tighter lower bound, with a probabilistic correctness guarantee derived using Chernoff's bound.

\begin{lemma}
\label{lemma:lb_ideal}
Let $S \subseteq \{0,1\}^n, f \in [0,1/2],$ and for each $m \in \{1, 2, \ldots, n\}$, let hash function $h_m$ be drawn randomly from $\mathcal{H}^f_{m \times n}$. Then,
\begin{align}
\left|S\right| & \geq \max_{m=1}^n \ 2^m \Pr[S(h_m) \geq 1].
\end{align}
\end{lemma}

Our theoretical lower bound is $L=2^{m}\mathbb \Pr\left[S(h)\geq1\right]$, which satisfies $L\leq |S|$ by the previous Lemma. In practice we cannot compute $\Pr[S(h)\geq 1]$ with infinite precision, so our practical lower bound is $\hat{L}=2^{m}\Pr_\text{est}\left[S(h)\geq1\right]$, \stefano{where $\hat{L}$ is a random variable} which will be defined in a moment. We would like to have a statement of the form $\Pr\left[\left|S\right|\geq \hat{L}\right]\geq 1-\delta$, \stefano{where the probability is with respect to the random variable $\hat{L}$}. It turns out that we can guarantee that $|S|$ is larger than the estimated lower bound shrunk by a $(1+\kappa)$ factor with high probability. Let $Y_{k}=\mathbb I\left[\left|h_{k}^{-1}(0)\cap S\right|\geq 1\right]$ and $Y = \sum_{k=1}^{T}Y_{k}.$ Let $\nu=\mathbb E\left[Y\right]=T\mathbb E\left[Y_{1}\right]=
%T\Pr\left[\left|h^{-1}(0)\cap S\right|\geq 1\right]=
T\Pr\left[S(h)\geq1\right].$ We define our estimator to be $\Pr_{\text{est}}\left[S(h)\geq1\right] = Y/T$.
%, where $h \in_R \mathcal{H}^f_{m \times n}$. 
Using Chernoff's bound, we have the following result.

\begin{theorem}
\label{thm:tighter-LB}
Let $\kappa > 0$. If $\Pr_{\text{est}}\left[S(h)\geq1\right] \geq c$, then
\begin{align*}
\Pr\left[|S|\geq\frac{2^{m} c}{(1+\kappa)}\right] \geq 1 - \exp\left(-\frac{\kappa^2 cT}{(1+\kappa)(2+\kappa)} \right).
\end{align*}
\end{theorem}


% \begin{proposition}
% With the notations defined in the previous paragraph, if $Y>c T$
% \begin{align}
% &\nonumber\Pr\left[|S|\geq\frac{2^{m}\Pr_{\mathrm{est}}\left[S(h)\geq1\right]}{(1+\epsilon)}\right]\geq\\
% &\qquad 1-\exp\left(-\frac{\epsilon^{2}T}{2+\epsilon}\mathbb{P}\left[S(h)\geq1\right]\right).
% \end{align}
% \end{proposition}

% \begin{proof}
% By the Chernoff bound, for $\epsilon>0$, we have
% \begin{align*}
% &\Pr\left[2^{m}\Pr_{\text{est}}\left[S(h)\geq1\right]= 2^{m}\frac{Y}{T}\geq2^{m}(1+\epsilon)\mathbb P\left[S(h)\geq1\right]\right]\notag\\
% &\leq\exp\left(-\frac{\epsilon^{2}T}{2 + \epsilon}\mathbb P\left[S(h)\geq1\right]\right).
% \end{align*}

% But since $2^{m}(1+\epsilon)\mathbb P\left[S(h)\geq1\right]\leq(1+\epsilon)\left|S\right|,$  we have
% \begin{align*}
% &\mathbb P\left[2^{m}\mathbb P_{\text{\text{est}}}\left[S(h)\geq1\right]
% \geq (1+\epsilon)|S|\right]\\
% &\leq\exp\left(-\frac{\epsilon^{2}T}{2 + \epsilon}\mathbb P\left[S(h)\geq1\right]\right),
% \end{align*}
% which completes the proof.
% \end{proof}

% Thus, to show that $|S|\geq \frac{2^m \Pr_\text{est}[S(h)\geq 1]}{(1 + \epsilon)}$ with probability at least $1 - \delta$, if $\Pr[S(h)\geq1] > c,$ the minimum number of samples is
% \begin{equation}
% T\geq\frac{\log\left(1/\delta\right)(2+\epsilon)}{c\epsilon^{2}}.
% \end{equation}


%%%%%%%%%%%%
\subsection{New Upper Bound for $|S|$}

%Empirical upper bound for the finches data set based
%on the above and on the \char`\"{}blue curve\char`\"{} (i.e., f{*}
%expression) from the ICML-2014 paper.
The upper bound expression for $f$ that we derive next is based on the contrapositive of the observation of \namecite{ermon2014low} that the larger $|S|$ is, the smaller an $f$ suffices to shatter it.
%\begin{lemma}
%If $\P\left[S=0\right]<1,$ then
%\begin{equation}
%\sigma_{S}>\sqrt{\frac{\P\left[S=0\right]}{1-%\P\left[S=0\right]}}\mu_{S}.
%\end{equation}
%\end{lemma}

For $n, m, f,$ and $\epsilon(n,m,q,f)$ from \cite{ermon2014low} 
%(also defined in Appendix, cf. Definition~\ref{def:wstar-etc})
, define:
%
\begin{align}
\label{def:vq}
v(q)=\frac{q}{2^{m}}\left(1+\epsilon(n, m, q, f)\cdot(q-1)-\frac{q}{2^{m}}\right)
\end{align}
This quantity is an upper bound on the variance $\mathrm{Var}[S(h)]$ of the number of surviving solutions as a function of the size of the set $q$, the number of constraints used $m$, and the statistical quality of the hash functions, which is controlled by the constraint density $f$. The following Lemma characterizes the asymptotic behavior of this upper bound on the variance:
%
\begin{lemma}
\label{lemma:inc}
$q^2/v(q)$ is an increasing function of $q$.
\end{lemma}

Using Lemma \ref{lemma:inc}, we are ready to obtain an upper bound on the size of the set $S$ in terms of the probability $\Pr[S(h) \geq 1]$ that at least one configuration from $S$ survives after adding the randomly generated constraints. 
\begin{lemma}
\label{upperb:lemma}
Let $S \subseteq \{0,1\}^n$ and $h \in_R \mathcal{H}^f_{m \times n}$.
 Then 
\[
%|S| \leq \min_x \left\{x \mid 1 - \frac{v(x)}{v(x)+\left(\frac{x}{2^m}\right)^2}  > \Pr[S(h) \geq 1]\right\}
|S| \leq \min \left\{z \mid \frac{1}{1 + 2^{2m} v(z) / z^2}  > \Pr[S(h) \geq 1]\right\}
\]
\end{lemma}

The probability $\Pr[S(h) \geq 1]$ is unknown, but can be estimated from samples. In particular, we can draw independent samples of the hash functions and get accurate estimates using Chernoff style bounds. We get the following theorem:

\begin{theorem}
\label{thm:UB}
Let $S \subseteq \{0,1\}^n$. Let $\Delta \in (0,1)$. Suppose we draw $T=24 \ln \frac{1}{\Delta}$ hash functions $h_1, \cdots, h_T$ from $\mathcal{H}^f_{m \times n}$.
If
$
\mathrm{Median}(\I[S(h_1)=0], \cdots, \I[S(h_T)=0])=0
$
then
\[
|S| \leq \min \left\{z \mid 1 - \frac{1}{1 + 2^{2m} v(z) / z^2} \geq \frac{3}{4}\right\}
\]
with probability at least $1-\Delta$.
\end{theorem}

% \begin{proof}
% If $|S| > \min_x \left\{x : 1 - \frac{v(x)}{v(x)+\left(\frac{x}{2^m}\right)^2}  \geq \frac{3}{4}\right\}$ then from Chernoff bound
% \begin{eqnarray*}
% %P[S(h_1)=0 \cap \cdots \cap S(h_T)=0] \leq \left(\frac{1}{4}\right)^T
% \Pr[\mathrm{Median}(\I[S(h_1)=0], \cdots, \I[S(h_T)=0])=0] \leq\\
% \exp\left(-\frac{T}{24}\right) \leq \alpha
% \end{eqnarray*}
% \end{proof}
This theorem provides us with a way of computing upper bounds on the cardinality of $S$ that hold with high probability. The bound is known to be tight (matching the lower bound derived in the previous section) if the family of hash function used is fully pairwise independent, i.e. $f=0.5$. 


==> sparse_count.tex <==
\subsection{Preliminaries: Counting by Hashing}

Let $S \subseteq \{0,1\}^n$ be a large, high-dimensional set. We are interested in computing $|S|$, the number of elements in $S$, when $S$ is defined succinctly through conditions or constraints that the elements of $S$ satisfy and membership in $S$ can be tested using an NP oracle. It has been shown \cite{wishicml13,cav13,mbound} that one can reliably estimate $|S|$, both in theory and in practice, by repeating the following simple process: randomly partition $S$ into $2^m$ cells for an appropriate $m \leq n$, uniformly randomly select one of these lower-dimensional cells, and compute whether $S$ has at least $p \geq 1$ elements in this cell. This can be accomplished with $p$ queries to an NP oracle.

While earlier work relied on Strongly Universal and Pairwise Independent families of hash functions for obtaining provable correctness guarantees, \citet{ermon2014low} showed that the weaker notion of Average Universal hash functions suffices for the purposes of hashing based counting. In particular, $f$-sparse hash functions (defined next), for sufficiently large $f < 1/2$, were shown to be Average Universal. and can also give probable correctness guarantees.

\begin{mydef}[\cite{ermon2014low}]
\label{def:sparse-hash}
Let $A\in \{0,1\}^{m \times n}$ be a random matrix whose entries are Bernoulli i.i.d.\ random variables of parameter $f \leq 1/2$, i.e., $\Pr[A_{ij}=1] = f$. Let $b \in \{0,1\}^m$ be chosen uniformly at random, independently from $A$. Then, $\mathcal{H}^f_{m \times n}=\{h_{A,b}: \{0,1\}^n \rightarrow \{0,1\}^m\}$, where $h_{A,b}(x)= A x + b \mod{2}$ and $  \in \mathcal{H}^f$ is chosen randomly according to this process, is a family of \emph{$f$-sparse hash functions}.
\end{mydef}

To facilitate discussion, we also define $S(h) = |\{x \in S \mid Ax+b = 0\}|$ to be the random variable indicating how many elements of $S$ \emph{survive} $h$.

If $\mathcal{H}^f_{m \times n}$ has the property that something in $S$ ``survives" with probability at least $1 - 1/\delta$, then as long as $\delta$ is bounded away from $2$ (e.g., $\delta = 9/4$), we can repeat the process $T$ times and use standard randomness amplification techniques to guarantee that something in $S$ survives at least $T/2$ times with a high probability, arbitrarily close to $1$.


Based on the intuition above, we give a hashing based counting procedure (Algorithm~\ref{algo}, SPARSE-COUNT), which relies on an NP oracle for $S(h)$  and is adapted from the SPARSE-WISH algorithm of \citet{ermon2014low}. Then we proceed to discuss its properties. In Theorem~\ref{thm:const} we show a necessary and sufficient condition so that SPARSE-COUNT may produce a constant factor approximation. Next in Theorem~\ref{thm:wish} we give a exact formula for the $f^*$ sufficient to satisfy the conditions of Theorem~\ref{thm:const}. Finally in  Theorem~\ref{thm:asymp} we give the asymptotic bound for $f^*$ necessary and sufficient to satisfy the conditions of Theorem~\ref{thm:const}

\begin{algorithm}[tb]
\caption{SPARSE-COUNT $(\text{oracle for\ } S, n, \Delta, \alpha)$ 
}
\label{algo_wish}
\begin{algorithmic}
\STATE $T \leftarrow \left\lceil \frac{\ln \left(1/\Delta\right)}{\alpha} \ln n \right\rceil$
\shengjia{I don't think this is related to n, I have found this to be $\frac{\ln(1/\Delta)}{\alpha}$}
\STATE $i=0$
\WHILE {$i \leq n$}
  \FOR {$t=1, \cdots, T$}
    \STATE $f^\ast = \min \{f | \epsilon(n,i,2^{i+2},f) < \frac{31}{5(2^{i+2}-1)} \}$
    \STATE $h^i_{A,b} \leftarrow$ hash function sampled from $\mathcal{H}^{f\ast}_{i \times n}$
    \STATE $w_i^t \leftarrow \mathbb{I}[S(h^i_{A,b}) \geq 1]$
  \ENDFOR
  \IF {$\mathrm{Median}(w_i^1, \cdots, w_i^T) < 1$}
    \STATE $\mathrm{break}$
  \ENDIF
\ENDWHILE
\STATE Return $2^{i}$
\shengjia{This is changed from $2^{i-1}$ to $2^{i}$, I think this gives better constant factor to our bound}
\end{algorithmic}
\end{algorithm}

\begin{theorem}
\label{thm:const}
For any $c > 0$, the necessary and sufficient condition for SPARSE-COUNT to give a constant factor $2^c$-approximation is that there $\exists \delta > 2$, so that \\
1. for the hashing family $\mathcal{H}^f_{(m-1) \times n}$ and an arbitrary set $S$ of size $2^{m - c}$
\[ Pr[S(h) = 0] \geq 1 - \frac{1}{\delta} \]
2. for the hashing family $\mathcal{H}^f_{m \times n}$ and an arbitrary set $S$ of size $2 ^ {m + c}$
\[ Pr[S(h) \geq 1] \geq 1 - \frac{1}{\delta} \]
\end{theorem}

\shengjia{Maybe it make more sense to formulate this as hypothesis testing?}
By $2^c$-approximation, our meaning here is from the perspective of hypothesis testing. Namely, if the actual size of the set $|S| \not\in [2^{m-c}, 2^{m+c}]$, the algorithm produces the output $2^m$ with probability less than a user specified $\Delta$. Therefore, we can reject the hypothesis $|S| \not\in [2^{m-c}, 2^{m+c}]$, and accept the alternative $|S| \in [2^{m-c}, 2^{m+c}]$ with arbitrarily high confidence $1 - \Delta$. \par 

We give a informal proof of why this theorem is correct. This is similar in spirit to the formal proof in \cite{wishicml13} of a similar problem. We call each step in the inner loop, which generates a parity constraints with m variables and inspects whether a bin is empty, a trial. If the bin is empty, we say the trial fails, otherwise it succeeds. If Algorithm 1 produces the result $2^m$, then more than half of the trials with $m-1$ constraints are successful, while at least half of the trials with $m$ constraints fail. If the condition of Theorem~\ref{thm:const} is satisfied: \par  
1. If $|S| < 2^{m - c}$, then with $m-1$ constraints, each trial $X_i$ only succeeds with probability $\frac{1}{\delta}$, For half of the $T$ trials to succeed, the probability is upper bounded by:
\[ \begin{aligned}
	& Pr\left\lbrace \sum_{i=1}^{T} X_i \geq \frac{T}{2} \right\rbrace \\
    =& Pr\left\lbrace \sum_{i=1}^{T} X_i \geq \frac{T}{\delta} \left(1 + \left(\frac{\delta}{2} - 1 \right)\right) \right\rbrace \\
    \leq& e^{-\frac{\left(\left(\delta/2 - 1 \right)\right)^2}{1 + \delta/2} 
    \frac{T}{\delta} } 
    = e^{-\frac{(\delta - 2)^2}{2\delta^2 + 4\delta}T}
\end{aligned} \]
For the confidence to be at least $\Delta$ we only need $\frac{2\delta^2 + 4\delta}{(\delta - 2)^2}\ln(1/\Delta)$ samples, which is a constant.

2. If $|S| > 2^{m + c}$, then with m constraints, each trial only fails with probability $\frac{1}{\delta}$, For half of the $T$ trials to fail, the probability is upper bounded in exactly the same way with the same amount of required samples

In the above theorem, the first condition is trivially satisfied for $c > 2$. Intuitively this is because to distribute $2^{m - c}$ elements into $2^{m-1}$ bins, at most $\frac{1}{2^{c-1}}$ of the bins can be non-empty. Formally, we have
\[ \begin{aligned}
	Pr[S(h) > 0] &= \sum_{A, b} \mathbb{I}[S(h_{A, b}) > 0]Pr[A]Pr[b] \\
    & \leq \sum_{A} \frac{2^{m - c}}{2^{m - 1}} Pr[A] = \frac{1}{2^{c-1}}
    \end{aligned}\]
    
The second condition requires careful derivation. \citet{wishicml13} showed that the pairwise independent family $\mathcal{H}^{1/2}_{m \times n}$ can satisfy this condition. Our interest in this paper, however, is in hash families with $f \ll 1/2$. We adapt the conclusions of \citet{ermon2014low} to give the following results

\begin{mydef}
\label{def:epsilon}
Let $n,m,q \in \mathbb{Z}^+, m,q \leq n, f \in [0,1/2],$ and $w^\ast = \max \left\{w \mid \sum_{j=1}^{w} \binom{n}{j} \leq q -1 \right\}$. Then,
%
\begin{align*}
\epsilon(n,m,q,f)  =  \frac{1}{q-1} \left( \sum_{w=1}^{w^\ast}\binom{n}{w} \left( \frac{1}{2} + \frac{1}{2} \left( 1-2f\right)^w \right)^m \right . \\
\left. +(q-1-\sum_{w=1}^{w^\ast}\binom{n}{w}) \left( \frac{1}{2} + \frac{1}{2} \left( 1-2f\right)^{w^\ast+1} \right)^m \right)
\end{align*}
%
\end{mydef}

\begin{theorem}[\cite{ermon2014low}]
\label{thm:wish}
Let $S \in \{0,1\}^n, m \leq n, \mu = |S|/2^m,$ and $f \in [0,1/2]$. If $\epsilon(n,m,|S|,f) \leq (\frac{\mu}{\delta-1} + \mu - 1)/(|S|-1)$ and $h \in_R \mathcal{H}^f_{m \times n}$, then $\Pr[S(h) \geq 1] \geq 1 - 1/\delta$.
\end{theorem}

Remarkably, even for $f < 1/2$ (i.e., without a family of pairwise independent hash functions), one can obtain, with a high probability, a constant factor approximation of the count as long as $f$ is large enough. This reflects a trade-off between statistical efficiency and computational complexity: while a larger $f$ leads to a hash family with better statistical guarantees, it also results in an increased computational burden on the oracle that tests whether $S(h^i_{A,b}) \geq 1$. 

In practice, it is most efficient to use the smallest possible $f$ that satisfies the condition in Theorem~\ref{thm:wish}, which is the $f^\ast$ computed by SPARSE-COUNT. 

==> sparse_count_legacy.tex <==
\section{Preliminaries: Counting by Hashing}
%\subsection{Counting by Hashing}

Let $x_1, \cdots, x_n$ be $n$ Boolean variables. Let $S \subseteq \{0,1\}^n$ be a large, high-dimensional set\footnote{We restrict ourselves to the binary case for the ease of exposition. Our work can be naturally extended to categorical variables.}. We are interested in computing $|S|$, the number of elements in $S$, when $S$ is defined succinctly through conditions or constraints that the elements of $S$ satisfy, and membership in $S$ can be tested using an NP oracle. For example, when $S$ is the set of solutions of a Boolean formula over $n$ binary variables, the problem of computing $|S|$ is known as model counting, which is the canonical $\#$-P complete problem~\cite{valiant1979complexity}.

In the past few years, there has been growing interest in approximate probabilistic algorithms for model counting. It has been shown \cite{mbound,wishicml13,cav13,achlioptasstochastic,belle2015hashing} that one can reliably estimate $|S|$, both in theory and in practice, by repeating the following simple process: randomly partition $S$ into $2^m$ cells and select one of these lower-dimensional cells, and compute whether $S$ has at least $p \geq 1$ elements in this cell (this can be accomplished with $p$ queries to an NP oracle). Somewhat surprisingly, repeating this procedure a small number of times provides a constant factor approximation to $|S|$ with high probability, even though counting problems (in $\#$-P) are believed to be harder than decision problems (in NP).

The correctness of the approach relies crucially on how the space is randomly partitioned into cells. 
All existing approaches partition the space into cells using parity or XOR constraints~\cite{mbound,cav13,ermon2014low,ivrii2015computing,achlioptasstochastic}. Specifically, the $2^m$ cells are defined by choosing $m$ subsets of variables, and defining the cells based on the parity of each subset of variables. Equivalently, one can generate $m$ parity (or XOR) constraints, and partition $S$ based on which parity constraints are satisfied. This can also be interpreted as a hash function, hashing the space into $2^m$ bins.

The way in which these constraints are generated affects the quality of the approximation of $|S|$ (the model count) obtained. Most methods \emph{randomly} generate $m$ parity constraints by adding each variable to each constraint with probability $f \leq 1/2$. 
%This construction is known to implement a Strongly Universal family of hash functions, and provides strong accuracy guarantees (constant factor approximation).  More generally, we have the following definition:
Formally,
\begin{mydef}[\cite{ermon2014low}]
\label{def:sparse-hash}
Let $A\in \{0,1\}^{m \times n}$ be a random matrix whose entries are Bernoulli i.i.d.\ random variables of parameter $f \leq 1/2$, i.e., $\Pr[A_{ij}=1] = f$. Let $b \in \{0,1\}^m$ be chosen uniformly at random, independently from $A$. Then, $\mathcal{H}^f_{m \times n}=\{h_{A,b}: \{0,1\}^n \rightarrow \{0,1\}^m\}$, where $h_{A,b}(x)= A x + b \mod{2}$ and $  \in \mathcal{H}^f$ is chosen randomly according to this process, is a family of \emph{$f$-sparse hash functions}.
\end{mydef}
Each function $h \in \mathcal{H}^f_{m \times n}$ partitions $\{0,1\}^n$ based on the following equivalence relation: $x_1 \sim x_2$ iff $h(x_1) = h(x_2)$. One can then select a cell $h^{-1}(y)$ by picking an element $y \in \{0,1\}^m$. To facilitate discussion, we also define $S(h) = |\{x \in S \mid h(x) = 0\}| = |S \cap h^{-1}(0)|$ to be the random variable indicating how many elements of $S$ \emph{survive} $h$, when $h$ is randomly chosen from $\mathcal{H}^f_{m \times n}$ as in Definition \ref{def:sparse-hash}. This is the number of elements of $S$ in the cell $h^{-1}(0)$. 

The idea to estimate $|S|$ is to define progressively smaller cells (by increasing $m$, the number of parity constraints used to define $h$), until no element of $S$ survives $h$. The intuition is that the larger $|S|$ is, the smaller the cells will have to be, and we can use this information to estimate $|S|$.
%If $\mathcal{H}^f_{m \times n}$ has the property that something in $S$ ``survives" with probability at least $3/4$, we can repeat the process $T$ times and use standard randomness amplification techniques to guarantee that something in $S$ survives at least $T/2$ times with a high probability, arbitrarily close to $1$.


Based on the intuition above, we give a hashing based counting procedure (Algorithm~\ref{algo}, SPARSE-COUNT), which relies on an NP oracle for $S(h)$  and is adapted from the SPARSE-WISH algorithm of \citet{ermon2014low}. Then we proceed to discuss its properties. In Theorem~\ref{thm:const} we show a 
%necessary and 
sufficient condition so that SPARSE-COUNT may produce a constant factor approximation of the size of any set $S$ (even if adversarially chosen). 
%Next in Theorem~\ref{thm:wish} we give a exact formula for the $f^*$ sufficient to satisfy the conditions of Theorem~\ref{thm:const}.
\stefano{define $\alpha$. in the pseudocode}

\begin{algorithm}[tb]
\caption{SPARSE-COUNT $(\text{oracle for\ } S, n, \Delta, \alpha, \mathcal{H}^{f}_{i \times n} )$ 
}
\label{algo}
\begin{algorithmic}[1]
\STATE $T \leftarrow \left\lceil \frac{\ln \left(1/\Delta\right)}{\alpha} \ln n \right\rceil$
\STATE $i=0$
\WHILE {$i \leq n$}
  \FOR {$t=1, \cdots, T$}
%    \STATE $f^\ast = \min \{f | \epsilon(n,i,2^{i+2},f) < \frac{31}{5(2^{i+2}-1)} \}$
    \STATE $h^i_{A,b} \leftarrow$ hash function sampled from $\mathcal{H}^{f}_{i \times n}$
    \STATE $w_i^t \leftarrow \mathbb{I}[S(h^i_{A,b}) \geq 1]$ \label{checkwithoracle}
  \ENDFOR
  \IF {$\mathrm{Median}(w_i^1, \cdots, w_i^T) < 1$}
    \STATE $\mathrm{break}$
  \ENDIF
\ENDWHILE
\STATE Return $2^{i-1}$
\end{algorithmic}
\end{algorithm}

\begin{theorem}[\cite{wishicml13}]
\label{thm:const}
The necessary and sufficient condition for SPARSE-COUNT to give a constant factor approximation is that for all $i$, when $h$ is chosen from $\mathcal{H}^f_{i \times n}$, there $\exists c > 0, \delta > 2$, so that  \\
1. for any set $S$ of size $2^{i - c}$
\[ Pr[S(h) = 0] \geq 1 - \frac{1}{\delta} \]
2. for any set $S$ of size $2 ^ {i + c}$
\[ Pr[S(h) \geq 1] \geq 1 - \frac{1}{\delta} \]
The approximation of $|S|$ is accurate up to a factor of $2^{2c }$ with probability at least $1-\Delta$.
\end{theorem}
In practice, line \ref{checkwithoracle} is implemented using a SAT solver as an NP-oracle. In a model counting application, this is accomplished by adding to the original formula $i$ parity constraints generated as in Definition \ref{def:sparse-hash} and checking for satisfiability. The procedure SPARSE-COUNT requires $O(n \log n)$ calls to a SAT solver.

The family $\mathcal{H}^{\frac{1}{2}}_{m \times n}$ (correspoding to XORs of average length $n/2$) is known to satisfy the assumptions of Theorem \ref{thm:const}. Unfortunately, checking satisfiability $S(h^i_{A,b}) \geq 1 $ (line \ref{checkwithoracle}) becomes increasingly harder as the length of the parity constraints increases~\cite{ghss07:shortxors,ermon2014low,ivrii2015computing,achlioptasstochastic}. For example, a parity constraint of length 1 simply freezes a variable. A constraint of length $k$, on the other hand, can only be propagated after $k-1$ variables have been set.

A natural question is therefore if the conditions of Theorem \ref{thm:const} are met by a family $\mathcal{H}^{f}_{m \times n}$ with $f<1/2$, as it would lead to shorter constraints and better runtime.
 
To gain some intuition, we observe that the first condition in Thm. \ref{thm:const} is trivially satisfied for $c > 1$ for any $0 < f \leq \frac{1}{2}$. Intuitively this is because to distribute $2^{m - c}$ elements into $2^m$ bins, at most $\frac{1}{2^c}$ of the bins can be non-empty. Formally, we have
\[ \begin{aligned}
	Pr[S(h) > 0] &= \sum_{A, b} \mathbb{I}[S(h_{A, b}) > 0]Pr[A]Pr[b] \\
    & \leq \sum_{A} \frac{2^{m - c}}{2^m} Pr[A] = \frac{1}{2^c}
    \end{aligned}\]
    
The second condition requires careful derivation. %\citet{wishicml13} showed that the pairwise independent family $\mathcal{H}^{1/2}_{m \times n}$ can satisfy this condition. Our interest in this paper, however, is in hash families with $f \ll 1/2$.  
Recently, \citet{ermon2014low} showed that the weaker notion of Average Universal hash functions suffices for the purposes of hashing based counting. In particular, $f^*$-sparse hash functions (defined next), for sufficiently large $f^* \lneqq 1/2$, were shown to be Average Universal, and hence give probable correctness guarantees.
We adapt the conclusions of \citet{ermon2014low} to give the following result

\begin{mydef}
\label{def:epsilon}
Let $n,m,q \in \mathbb{Z}^+, m,q \leq n, f \in [0,1/2],$ and $w^\ast = \max \left\{w \mid \sum_{j=1}^{w} \binom{n}{j} \leq q -1 \right\}$. Then,
%
\begin{align*}
\epsilon(n,m,q,f)  =  \frac{1}{q-1} \left( \sum_{w=1}^{w^\ast}\binom{n}{w} \left( \frac{1}{2} + \frac{1}{2} \left( 1-2f\right)^w \right)^m \right . \\
\left. +(q-1-\sum_{w=1}^{w^\ast}\binom{n}{w}) \left( \frac{1}{2} + \frac{1}{2} \left( 1-2f\right)^{w^\ast+1} \right)^m \right)
\end{align*}
%
\end{mydef}

\begin{theorem}[\cite{ermon2014low}]
\label{thm:wish}
Let $S \in \{0,1\}^n, m \leq n, \mu = |S|/2^m,$ and $f \in [0,1/2]$. If $\epsilon(n,m,|S|,f) \leq (\frac{\mu}{\delta-1} + \mu - 1)/(|S|-1)$ and $h \in_R \mathcal{H}^f_{m \times n}$, then $\Pr[S(h) \geq 1] \geq 1 - 1/\delta$.
\end{theorem}

Theorem \ref{thm:wish} provides a sufficient condition for obtaining constant factor approximations. specifically, it provides a value $f^*(n,m)$ such that if $f\geq f*$, the assumptions of Theorem \ref{thm:const} are met and one gets a constant factor approximation. \emph{Is it possible to do better?} We show that (asymptotically) it's not possible to improve over this result, i.e., use shorter constraints and meet the conditions of Theorem \ref{thm:const}.

==> sparse_count_new.tex <==
\section{Preliminaries: Counting by Hashing}
%\subsection{Counting by Hashing}

Let $x_1, \cdots, x_n$ be $n$ Boolean variables. Let $S \subseteq \{0,1\}^n$ be a large, high-dimensional set\footnote{We restrict ourselves to the binary case for the ease of exposition. Our work can be naturally extended to categorical variables.}. We are interested in computing $|S|$, the number of elements in $S$, when $S$ is defined succinctly through conditions or constraints that the elements of $S$ satisfy and membership in $S$ can be tested using an NP oracle. For example, when $S$ is the set of solutions of a Boolean formula over $n$ binary variables, the problem of computing $|S|$ is known as model counting, which is the canonical $\#$-P complete problem~\cite{valiant1979complexity}.

In the past few years, there has been growing interest in approximate probabilistic algorithms for model counting. It has been shown \cite{mbound,wishicml13,cav13,achlioptasstochastic,belle2015hashing} that one can reliably estimate $|S|$, both in theory and in practice, by repeating the following simple process: randomly partition $S$ into $2^m$ cells and select one of these lower-dimensional cells, and compute whether $S$ has at least 1 element in this cell (this can be accomplished with a query to an NP oracle, e.g., invoking a SAT solver). Somewhat surprisingly, repeating this procedure a small number of times provides a constant factor approximation to $|S|$ with high probability, even though counting problems (in $\#$-P) are believed to be significantly harder than decision problems (in NP).

The correctness of the approach relies crucially on how the space is randomly partitioned into cells. 
All existing approaches partition the space into cells using parity or XOR constraints. A parity constraint defined on a subset of variables checks whether an odd or even number of the variables take the value 1.
%~\cite{mbound,cav13,ermon2014low,ivrii2015computing,achlioptasstochastic}. 
%Specifically, the $2^m$ cells are defined by choosing $m$ subsets of variables, and defining the cells based on the parity of each subset of variables. 
Specifically, $m$ parity (or XOR) constraints are generated, and $S$ is partitioned into $2^m$ equivalence classes based on which parity constraints are satisfied.

The way in which these constraints are generated affects the quality of the approximation of $|S|$ (the model count) obtained. Most methods \emph{randomly} generate $m$ parity constraints by adding each variable to each constraint with probability $f \leq 1/2$. This construction can also be interpreted as defining a hash function, mapping the space $\{0,1\}^n$ into $2^m$ hash bins (cells).
%This construction is known to implement a Strongly Universal family of hash functions, and provides strong accuracy guarantees (constant factor approximation).  More generally, we have the following definition:
Formally,
\begin{mydef}
\label{def:sparse-hash}
Let $A\in \{0,1\}^{m \times n}$ be a random matrix whose entries are Bernoulli i.i.d.\ random variables of parameter $f \leq 1/2$, i.e., $\Pr[A_{ij}=1] = f$. Let $b \in \{0,1\}^m$ be chosen uniformly at random, independently from $A$. Then, $\mathcal{H}^f_{m \times n}=\{h_{A,b}: \{0,1\}^n \rightarrow \{0,1\}^m\}$, where $h_{A,b}(x)= A x + b \mod{2}$ and $ h_{A,b} \in_R \mathcal{H}_{m \times n}^f$ is chosen randomly according to this process, is a family of \emph{$f$-sparse hash functions}.
\end{mydef}
% Each function $h \in \mathcal{H}^f_{m \times n}$ partitions $\{0,1\}^n$ based on the following equivalence relation: $x_1 \sim x_2$ iff $h(x_1) = h(x_2)$. One can then select a cell $h^{-1}(y)$ by picking an element $y \in \{0,1\}^m$. To facilitate discussion, we also define $S(h) = |\{x \in S \mid h(x) = 0\}| = |S \cap h^{-1}(0)|$ to be the random variable indicating how many elements of $S$ \emph{survive} $h$, when $h$ is randomly chosen from $\mathcal{H}^f_{m \times n}$ as in Definition \ref{def:sparse-hash}. This is the number of elements of $S$ in the cell $h^{-1}(0)$. 

The idea to estimate $|S|$ is to define progressively smaller cells (by increasing $m$, the number of parity constraints used to define $h$), until the cells become so small that no element of $S$ can be found inside a (randomly) chosen cell. The intuition is that the larger $|S|$ is, the smaller the cells will have to be, and we can use this information to estimate $|S|$.
%If $\mathcal{H}^f_{m \times n}$ has the property that something in $S$ ``survives" with probability at least $3/4$, we can repeat the process $T$ times and use standard randomness amplification techniques to guarantee that something in $S$ survives at least $T/2$ times with a high probability, arbitrarily close to $1$.


Based on this intuition, we give a hashing-based counting procedure (Algorithm~\ref{algo_wish}, SPARSE-COUNT), which relies on an NP oracle $\mathcal{O}_S$ to check if $S$ has an element in the cell. It is adapted from the SPARSE-WISH algorithm of \citet{ermon2014low}. The algorithm takes as input $n$ families of \emph{$f$-sparse hash functions} $\{\mathcal{H}^{f_i}_{i \times n}\}_{i=0}^n$ which are used to partition the space into cells. In practice, line \ref{checkwithoracle} is implemented using a SAT solver as an NP-oracle. In a model counting application, this is accomplished by adding to the original formula $i$ parity constraints generated as in Definition \ref{def:sparse-hash} and checking the satisfiability of the augmented formula. 
%The procedure SPARSE-COUNT requires $O(n \ln n)$ calls to a SAT solver.
%Then we proceed to discuss its properties. 
% In the following Theorem~\ref{thm:const} we show a 
% %necessary and 
% \shengjia{I think this is necessary and sufficient}
% sufficient condition so that SPARSE-COUNT may produce a constant factor approximation of the size of any set $S$ (even if adversarially chosen). 
%Next in Theorem~\ref{thm:wish} we give a exact formula for the $f^*$ sufficient to satisfy the conditions of Theorem~\ref{thm:const}.
%\stefano{define $\alpha$. in the pseudocode}

\begin{algorithm}[tb]
\caption{SPARSE-COUNT $(\mathcal{O}_S, \Delta, \alpha, \{\mathcal{H}^{f_i}_{i \times n}\}_{i=0}^n )$ 
}
\label{algo_wish}
\begin{algorithmic}[1]
\STATE $T \leftarrow \left\lceil \frac{\ln \left(1/\Delta\right)}{\alpha} \ln n \right\rceil$
\STATE $i=0$
\WHILE {$i \leq n$}
  \FOR {$t=1, \cdots, T$}
%    \STATE $f^\ast = \min \{f | \epsilon(n,i,2^{i+2},f) < \frac{31}{5(2^{i+2}-1)} \}$
    \STATE $h^i_{A,b} \leftarrow$ hash function sampled from $\mathcal{H}^{f_i}_{i \times n}$
    \STATE Let $S(h^i_{A,b}) = |\{x \in S \mid h^i_{A,b}(x) = 0\}|$
    \STATE $w_i^t \leftarrow \mathbb{I}[S(h^i_{A,b}) \geq 1]$ \label{checkwithoracle}
  \ENDFOR
  \IF {$\mathrm{Median}(w_i^1, \cdots, w_i^T) < 1$}
    \STATE $\mathrm{break}$
  \ENDIF
  \STATE $i = i +1$
\ENDWHILE
\STATE Return $\lfloor 2^{i-1} \rfloor$
\end{algorithmic}
\end{algorithm}

% \shengjia{Maybe it make more sense to formulate this as hypothesis testing?}
% By $2^c$-approximation, our meaning here is from the perspective of hypothesis testing. Namely, if the actual size of the set $|S| \not\in [2^{m-c}, 2^{m+c}]$, the algorithm produces the output $2^m$ with probability less than a user specified $\Delta$. Therefore, we can reject the hypothesis $|S| \not\in [2^{m-c}, 2^{m+c}]$, and accept the alternative $|S| \in [2^{m-c}, 2^{m+c}]$ with arbitrarily high confidence $1 - \Delta$. \par 

% We give a informal proof of why this theorem is correct. This is similar in spirit to the formal proof in \cite{wishicml13} of a similar problem. We call each step in the inner loop, which generates a parity constraints with m variables and inspects whether a bin is empty, a trial. If the bin is empty, we say the trial fails, otherwise it succeeds. If Algorithm 1 produces the result $2^m$, then more than half of the trials with $m-1$ constraints are successful, while at least half of the trials with $m$ constraints fail. If the condition of Theorem~\ref{thm:const} is satisfied: \par  
% 1. If $|S| < 2^{m - c}$, then with $m-1$ constraints, each trial $X_i$ only succeeds with probability $\frac{1}{\delta}$, For half of the $T$ trials to succeed, the probability is upper bounded by:
% \[ \begin{aligned}
% 	& Pr\left\lbrace \sum_{i=1}^{T} X_i \geq \frac{T}{2} \right\rbrace \\
%     =& Pr\left\lbrace \sum_{i=1}^{T} X_i \geq \frac{T}{\delta} \left(1 + \left(\frac{\delta}{2} - 1 \right)\right) \right\rbrace \\
%     \leq& e^{-\frac{\left(\left(\delta/2 - 1 \right)\right)^2}{1 + \delta/2} 
%     \frac{T}{\delta} } 
%     = e^{-\frac{(\delta - 2)^2}{2\delta^2 + 4\delta}T}
% \end{aligned} \]
% For the confidence to be at least $\Delta$ we only need $\frac{2\delta^2 + 4\delta}{(\delta - 2)^2}\ln(1/\Delta)$ samples, which is a constant.

% 2. If $|S| > 2^{m + c}$, then with m constraints, each trial only fails with probability $\frac{1}{\delta}$, For half of the $T$ trials to fail, the probability is upper bounded in exactly the same way with the same amount of required samples

Typically, $\{\mathcal{H}^{\frac{1}{2}}_{i \times n}\}$ is used, corresponding to XORs where each variable is added with probability $1/2$ (hence with average length $n/2$). We call these \textbf{long parity constraints}. In this case, it can be shown that SPARSE-COUNT will output a factor $16$ approximation of $|S|$ with probability at least $1-\Delta$~\cite{ermon2014low}. Unfortunately, checking satisfiability $S(h^i_{A,b}) \geq 1 $ (line \ref{checkwithoracle}) can be very difficult when many long parity constraints are added to a formula~\cite{ghss07:shortxors,ermon2014low,ivrii2015computing,achlioptasstochastic}. For example, a parity constraint of length 1 simply freezes a variable. A constraint of length $k$, on the other hand, can only be propagated after $k-1$ variables have been set. From a theoretical perspective, parity constraints are known to be fundamentally difficult for the resolution proof system underlying SAT solvers, see for example the exponential scaling of Tseitin tautologies.
A natural question is therefore whether \textbf{short parity constraints} can be used in SPARSE-COUNT and provide reliable bounds for $|S|$.

% To facilitate discussion, we define $S(h) = |\{x \in S \mid h(x) = 0\}| = |S \cap h^{-1}(0)|$ to be the random variable indicating how many elements of $S$ \emph{survive} $h$, when $h$ is randomly chosen from $\mathcal{H}^f_{m \times n}$ as in Definition \ref{def:sparse-hash}. This is the number of elements of $S$ in the cell $h^{-1}(0)$. 
Intuitively, for the method to work we want the hash functions $\{\mathcal{H}^{f_i}_{i \times n}\}$ to have a small collision probability. In other words, we want to ensure that when we partition the space into cells, configurations from $S$ are divided into cells evenly. This gives a direct relationship between the original number of solutions $|S|$ and the (random) number of solutions in one (randomly chosen) cell, $S(h)$. More precisely, we say that the hash family \emph{shatters} $S$ if the following holds:
\begin{mydef}
\label{def:shatter}
For $\epsilon > 0$, a family of hash functions $\mathcal{H}^{f}_{i \times n}$ $\epsilon$-\emph{shatters} a set $S$ if $\Pr[S(h) \geq 1] \geq 1/2+\epsilon$ when $h \in_R \mathcal{H}^{f}_{i \times n}$, where $S(h) = |\{x \in S \mid h(x) = 0\}|$.
\end{mydef}
The crucial property we need to obtain reliable estimates is that the hash functions (equivalently, parity constraints) are able to shatter sets $S$ with arbitrary ``shape''. This property is both sufficient and necessary for SPARSE-COUNT to provide accurate model counts with high probability:
\begin{theorem}
\label{thm:const}
(Informal statement) A necessary and sufficient condition for SPARSE-COUNT to provide a constant factor approximation to $|S|$ is that each family $\mathcal{H}^{f_i}_{i \times n}$ $\epsilon$-shatters all sets $S'$ of size $|S'|=2^{i + c}$ for some $c\geq 2$.
\end{theorem}
A formal statement and proof is provided in the companion technical report~\cite{zhaotech}.
\begin{comment}
% \begin{theorem}
% \label{thm:const}
% (Sufficiency) Let $\{\mathcal{H}^{f_i}_{i \times n}\}_{i=0}^n$ be families of $f_i$-sparse hash functions. If there exists $c \geq 2$ and $\epsilon > 0$, such that for all $i$, $\mathcal{H}^{f_i}_{i \times n}$ $\epsilon$-shatters all sets $S' \subseteq \{0,1\}^n$ of size $|S'|=2^{i + c}$, then for any set $S$, $0<\Delta<1$, and $\alpha \leq 2(\min(\epsilon,1/2-1/2^c))^2\ln 2$, SPARSE-COUNT$(\mathcal{O}_S, \Delta, \alpha, \{\mathcal{H}^{f_i}_{i \times n}\} )$ outputs a $2^{c+1}$ approximation of $|S|$
% % \[
% % \frac{|S|}{2^{c}} \leq SPARSE-COUNT (\mathcal{O}_S, \Delta, \alpha, \{\mathcal{H}^{f_i}_{i \times n}\} ) \leq |S|2^{c}
% % \]
% with probability at least $1-\Delta$. (Necessity) If there exists an $i$ and a set $S$ of size $2^{i+c}$ such that for all $\epsilon>0$ $\mathcal{H}^{f_i}_{i \times n}$ does not $\epsilon$-shatter $S$, then for any choice of $\alpha>0$ and $0<\Delta<1$, SPARSE-COUNT$(\mathcal{O}_S, \Delta, \alpha, \{\mathcal{H}^{f_i}_{i \times n}\} )$ outputs a $2^c$ approximation of $|S|$
% with probability at most $1/2$.

% \end{theorem}
% \begin{proof}
% proof of the necessity part.
% We choose $S=S'$. Let's condition on the event that the outer loop reaches iteration $i$. For any $T \geq 1$ (therefore, for any choice of $\Delta$ and $\alpha$), the while loop breaks with probability at least $1/2$. Therefore, the output satisfies $\frac{|S|}{2^{c}} \leq SPARSE-COUNT(\mathcal{O}_S, \Delta, \alpha, \{\mathcal{H}^{f_i}_{i \times n}\})$ with probability at most $1/2$.
% \end{proof}

% To gain some intuition, we observe that the first condition is trivially satisfied for $c > 2$. Intuitively this is because to distribute $2^{m - c}$ elements into $2^{m-1}$ bins, at most $\frac{1}{2^{c-1}}$ of the bins can be non-empty. Formally, we have
% \[ \begin{aligned}
% 	Pr[S(h) > 0] &= \sum_{A, b} \mathbb{I}[S(h_{A, b}) > 0]Pr[A]Pr[b] \\
%     & \leq \sum_{A} \frac{2^{m - c}}{2^{m - 1}} Pr[A] = \frac{1}{2^{c-1}}
%     \end{aligned}\]
    
%The second condition requires careful derivation. %\citet{wishicml13} showed that the pairwise independent family $\mathcal{H}^{1/2}_{m \times n}$ can satisfy this condition. Our interest in this paper, however, is in hash families with $f \ll 1/2$.  

We adapt the conclusions of \citet{ermon2014low} to give the following result
\begin{mydef}
\label{def:epsilon}
Let $n,m,q \in \mathbb{Z}^+, m,q \leq n, f \in [0,1/2],$ and $w^\ast = \max \left\{w \mid \sum_{j=1}^{w} \binom{n}{j} \leq q -1 \right\}$. Then,
%
\begin{align*}
\epsilon(n,m,q,f)  =  \frac{1}{q-1} \left( \sum_{w=1}^{w^\ast}\binom{n}{w} \left( \frac{1}{2} + \frac{1}{2} \left( 1-2f\right)^w \right)^m \right . \\
\left. +(q-1-\sum_{w=1}^{w^\ast}\binom{n}{w}) \left( \frac{1}{2} + \frac{1}{2} \left( 1-2f\right)^{w^\ast+1} \right)^m \right)
\end{align*}
%
\end{mydef}

\begin{theorem}[\cite{ermon2014low}]
\label{thm:wish}
Let $S \in \{0,1\}^n, m \leq n, \mu = |S|/2^m,$ and $f \in [0,1/2]$. If $\epsilon(n,m,|S|,f) \leq (\frac{\mu}{\delta-1} + \mu - 1)/(|S|-1)$ and $h \in_R \mathcal{H}^f_{m \times n}$, then $\Pr[S(h) \geq 1] \geq 1 - 1/\delta$.
\end{theorem}
\end{comment}
Long parity constraints, i.e., $1/2$-sparse hash functions, are capable of shattering sets of arbitrary shape. When $h \in_R \mathcal{H}^{\frac{1}{2}}_{i \times n}$, it can be shown that configurations $x\in \{0,1\}^n$ are placed into hash bins (cells) pairwise independently, and this guarantees shattering of sufficiently large sets of arbitrary shape.   Recently, \citet{ermon2014low} showed that sparser hash functions can be used for approximate counting as well. In particular, $f^*$-sparse hash functions, for sufficiently large $f^* \lneqq 1/2$, were shown to have good enough shattering capabilities.
% Theorem \ref{thm:wish} provides a sufficient condition for obtaining constant factor approximations. specifically, it provides a value $f^*(n,m)$ such that if $f\geq f^*$, the assumptions of Theorem \ref{thm:const} are met and one gets a constant factor approximation. 
It is currently not known whether $f^*$ is the optimal constraint density.
%\emph{Is it possible to do better, and what is the optimal constraint density?}
%We show that (asymptotically) it's not possible to improve over this result, i.e., use shorter constraints and meet the conditions of Theorem \ref{thm:const}.


